LSTM for Model-Based Anomaly Detection in Cyber-Physical Systems

Anomaly detection is the task of detecting data which differs from the normal behaviour of a system in a given context. In order to approach this problem, data-driven models can be learned to predict current or future observations. Oftentimes, anomalous behaviour depends on the internal dynamics of the system and looks normal in a static context. To address this problem, the model should also operate depending on state. Long Short-Term Memory (LSTM) neural networks have been shown to be particularly useful to learn time sequences with varying length of temporal dependencies and are therefore an interesting general purpose approach to learn the behaviour of arbitrarily complex Cyber-Physical Systems. In order to perform anomaly detection, we slightly modify the standard norm 2 error to incorporate an estimate of model uncertainty. We analyse the approach on artificial and real data.

==> anomaly.tex <==
\section{Anomaly Detection}
To discriminate between normal and anomalous data, we can calculate the normalized residuals $r_t=\frac{y_t^i-\mu_t^i}{\sigma_t^i}$. At this point, given that the distribution for the random variable is known to be normal:
\begin{equation}
    p(r_t|s_{t-1},x_t)=\mathcal{N}(r_t,1),
\end{equation}
an arbitrary (number of) statistical tests can be performed in order to classify the point as anomalous or not. It is possible to combine several samples and/or features and then analyse the aggregate statistics. Alternatively one could threshold the normal distribution given the test point $r_t$. The threshold can either be learned (as is often done in the literature [..]) on the training or held out data to include a specified percentile of the training data (e.g. 100\%) or calculated to include a specified percentile of the expected distribution, as is done in the following.\\
The probability of obtaining a measurement $r=R$ as unexpected as seen or even less expected is given by integrating the tails of the normal distribution outside $\pm R$ from the mean:
\begin{equation}
    P(|r|>R)=2\int_R^\infty\mathcal{N}(r)\textrm{d}r=\int_{R^2}^\infty\textrm{PDF}_{\chi^2}(r;1)\textrm{d}r
\end{equation}
where $\textrm{PDF}_{\chi^2}(x;k)$ is the probability density of the square sum of $k$ independent variables. In case one decides to threshold the P-value, thereby classifying everything below as anomalous, it directly corresponds to the expected False Positive rate. Exemplary thresholds for $r$ are summarized in table \ref{tab:my_label}.
\begin{table}[!ht]
    \centering
    \begin{tabular}{c|ccccc}
        $R$ & 1 & 2 & 3 & 4 & 5 \\
        \hline
        $P(|r|>R)$ & 0.317 & $4.6\cdot10^{-2}$ & $2.7\cdot10^{-3}$ & $6.3\cdot10^{-5}$ & $5.7\cdot10^{-7}$
    \end{tabular}
    \caption{Expected false positive rate when thresholding $r>R$ to be classified as anomalous (positive)}
    \label{tab:my_label}
\end{table}
This is the expected frequency of points sampled from a normal distribution to be  classified as anomalous. Of course, anomalous points themselves are not expected to be distributed normally and thus should exceed the threshold value much more frequently.\\
The strength of this approach is that it is not necessary to learn the threshold with held out data, possibly containing known anomalies. Instead, it is not necessary at all to have ever measured an anomaly, exact statements about the expected frequency of false positives can be made and thresholds can be chosen according to ones preferences given the test data size and desired sensitivity.

==> genesis.tex <==
\red{\subsection{Pick and Place demonstrator}}\label{subsec:genesis}

The \red{\textit{Genesis}} pick-and-place demonstrator is a portable machine sorting small metallic and non-metallic blocks of material into two different boxes. It runs through different stages of picking up material, transporting it to an inductive sensor and putting it into a corresponding box.

Input signals will consist of several binary readings confirming the motor reached certain positions, material ejection signals as well as a variable confirming that a metallic material has been detected.
Output signals contain the motor current, velocity, position and acceleration as it is moving the material around.

==> method.tex <==
\section{Idea}
The task is to describe and monitor a dynamic physical system. The system exhibits a cyclic behaviour and has some internal and non-observed state that keeps track of both progress within each cycle and possible additional information of different kinds working modes. The system is partly influenced by external factors such as environmental, cybernetic, human or random dependencies. This can entail control variables such as a starting signal to a machine. All of this information can be summarized into a data structure which contains the known causal variables: $\mathbf{x}_t\in\mathbb{R}^n$; $n\in\mathbb{N}$, one for each point in time $t$.

Measurements on the system can be performed and are highly dependent on its state. The observations on the system are summarized in the vector: $\mathbf{y}_t\in\mathbb{R}^m$; $m\in\mathbb{N}$.

We will join all the information that exists and influences the system in its state $s_t\in\mathcal{S}$ where $\mathcal{S}$ is the set of all possible system states.

Notice, that given a system state $s_t$, the observables $\mathbf{y}_t$ are either uniquely determined (zero entropy) or exhibit some leftover noise which is characteristic to each variable. If the latter applies, the noise itself is assumed to be of pure gaussian nature. To see this, recall that the normal distribution maximizes the entropy for a real valued random variable given the constraints of zero mean and unit variance. It therefore contains no information by its very nature and the assumption of all to $\mathbf{y}$ relevant information being included in the hidden state representation $s_t$ is then satisfied.\\
%This separation is not always absolutely clear, however, both observables $\mathbf{x}$ and $\mathbf{y}$ can be summarized to be drawn independently from a joint distribution $p(x_t,y_t|s_t)$ given some hidden state $s$ at time $t$. All information that possibly exists and influences the system is included in this variable. Thus, the observables $x$ or $y$ are either uniquely determined given the state of the system (zero entropy) or exhibit some leftover noise characteristic to each variable.
The task will be to model both $\mathbf{y}_t$ and $s_t$ given the information about the state that is given in the time sequence of the variable $\mathbf{x}$. $\mathbf{y}_t$ is assumed to be distributed normally with mean $\mathbf{\mu}_t$ and variance $V_t$:
\begin{equation}
    p(\mathbf{y}_t|\mathbf{x}_t,s_{t-1})=\left(2\pi\right)^{-M/2}\left|V_t\right|^{-\frac{1}{2}}\exp\left(-\frac{1}{2}\left(y_t-\mu_t\right)^T V^{-1}_t\left(y_t-\mu_t\right)\right)
\end{equation}
Furthermore, because all information is in the state variable, all elements of $y_t^{i}\in \mathbf{y}_t$ are conditionally independent from each other given $\mathbf{x}_t$ and $s_t$. In a real physical system, this corresponds to the fact, that two sensors might take measurements within the same environment and therefore are (possibly maximally) correlated, but given the \textit{complete} internal state of the system, the remaining noise on each sensor is independent from each other (In a similar way, the noise of the same sensor is assumed to be independent of itself for different times, i.e $y_t^{i}$ and $y_{t'}^{i}$, $t\neq t'$). $V_t$ is therefore diagonal and $p(\mathbf{y}_t|\mathbf{x}_t,s_t)$ factorizes to the following expression:
\begin{equation}
    p(\mathbf{y}_t|\mathbf{x}_t,s_{t-1})=\prod_{i=0}^{m}\left(2\pi\left(\sigma^{i}_t\right)^2\right)^{-\frac{1}{2}}\exp\left\{-\frac{1}{2}\left(\frac{y_t^i-\mu_t^i}{\sigma_t^i}\right)^2\right\}\label{eq:likelihood}
\end{equation}
The problem is therefore reduced to finding a mapping of the form:
\begin{equation}
    f: \mathbf{x}_t,s_{t-1} \rightarrow \mathbf{\mu}_t, \mathbf{\sigma}_t
\end{equation}
Where $\mathbf{\sigma}_t$ is the vector with elements $\left\{\sigma_t^i; i\in\mathbb{N}_0<m\right\}$. However, given that the system state is not actually measured in a real physical system, it is not possible to find such a mapping directly. 
Instead we will model the system state as well, inferred from the different modes of observations made on the system as well as the inter dependencies of the variables $\mathbf{x}_t$ and $\mathbf{y}_t$. By doing so, we will implicitly model the time variance of the system. We denote the modelled system state as $\mathbf{s}_t\in\mathbb{R}^k$. The desired mapping now has the form:
\begin{equation}
    f: \mathbf{x}_t, \mathbf{s}_{t-1} \rightarrow \mathbf{s}_{t}, \mathbf{\mu}_t, \mathbf{\sigma}_t
\end{equation}
We will employ a Long Short Term Memory network to find $f$ and model all of the $\mu_t$, $\sigma_t$ (short term memory state) \emph{as well} as the hidden state $s_t$ (as its internal long term memory states) and use supervised learning on the targets $y_t$ with stochastic gradient descent to train the weights of the parametric function. Maximizing the likelihood function (\ref{eq:likelihood}) is equivalent to minimizing the negative log likelihood loss function:
\begin{equation}
    L_t=\sum_i\left[\left(\frac{y_t^i-\mu_t^i}{\sigma_t^i}\right)^2+2\log\sigma_t^i\right]
\end{equation}
Writing $\sigma_t^i=\exp(\tau_t^i)$ guarantees $\sigma>0$ and provides numerical stability in the learning process. The network architecture consists of several (1-5) fully recurrent stacked LSTM layers with a subsequent fully connected tanh activation neural network with $2m$ output channels, one for each $y^i$ and $\tau^i$. Gradients are truncated in time after $t_{\textrm{\small{max}}}$ steps, typically between 5 and 50.\\
In the learning stage the neural net will optimize its weights in order to model the domain dependent functions $\mu(\mathbf{x}_t,\mathbf{s}_t)$ and $\sigma(\mathbf{x}_t,\mathbf{s}_t)$ as accurate as possible. Put differently, the neural net learns the \textit{domain mean}, taking for each known state the average over the known observations falling into that category. The method is therefore completely self regularizing as long as \textit{enough} data exists for each domain to determine sensible mean and standard deviation values.
\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth]{pfg_valid.png}
    \caption{Three artificial signals learned jointly with an LSTM network. The signal (yellow) is sampled with different noise levels at different domains. The LSTM is able to learn both mean (blue) as well as standard deviation (shaded) given as input a periodic signal of all 0 and one 1 at the start of each period.}
    \label{fig:sim_signals}
\end{figure}
